Formal Verification of Usage Control Models: A Case Study of UseCON Using TLA+

Usage control models provide an integration of access control, digital rights, and trust management. To achieve this integration, usage control models support additional concepts such as attribute mutability and continuity of decision. However, these concepts may introduce an additional level of complexity to the underlying model, rendering its definition a cumbersome and prone to errors process. Applying a formal verification technique allows for a rigorous analysis of the interactions amongst the components, and thus for formal guarantees in respect of the correctness of a model. In this paper, we elaborate on a case study, where we express the high-level functional model of the UseCON usage control model in the TLA+ formal specification language, and verify its correctness for <=12 uses in both of its supporting authorisation models.

==> eptcsdata.tex <==
\providecommand{\firstpage}{52}
\providecommand{\publicationstatus}{Simon Bliudze and Saddek Bensalem (Eds):\\
Methods and Tools for Rigorous System Design (MeTRiD 2018)\\
EPTCS 272, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.272.5}{10.4204/EPTCS.272.5}}
\pdfoutput=1

